Secret Sharing based Secure Regressions with Applications

Nowadays, the utilization of the ever expanding amount of data has made a huge impact on web technologies while also causing various types of security concerns. On one hand, potential gains are highly anticipated if different organizations could somehow collaboratively share their data for technological improvements. On the other hand, data security concerns may arise for both data holders and data providers due to commercial or sociological concerns. To make a balance between technical improvements and security limitations, we implement secure and scalable protocols for multiple data holders to train linear regression and logistic regression models. We build our protocols based on the secret sharing scheme, which is scalable and efficient in applications. Moreover, our proposed paradigm can be generalized to any secure multiparty training scenarios where only matrix summation and matrix multiplications are used. We demonstrate our approach by experiments which shows the scalability and efficiency of our proposed protocols, and finally present its real-world applications.

==> section/algorithm.tex <==
\section{Secure Matrix Multiplication Protocols}\label{sec-algo}
As emphasized in Section \ref{sec-hor}, the protocol for the horizontally partitioned data scenario highly depends on a `black-box' protocol which can implement the functionality that two parties each holding a matrix collaboratively compute the resulting product of their individual inputs.

We design two protocols for two party secure matrix multiplication, as is shown in Algorithm \ref{algo-trust} and Algorithm \ref{algo-ssmm}. Algorithm \ref{algo-trust} is based on a classical implementation with trusted initializer, while in Algorithm \ref{algo-ssmm} we bypass the trusted initializer by sacrificing some security guarantee. We will analyze both algorithms and theoretically prove the correctness and security.

\subsection{Simulation-based Security Proof}
To formally prove that a protocol is secure, we adopt the \textit{semi-honest} point of view, in which each participant of the protocol truthfully obeys the protocol while being curious about the other parties' original data. Under the simulation-based proof, whatever can be computed by one party can be simulated given only the messages it receives during the protocol, which implies that each party learns nothing from the protocol execution beyond what they can derive from messages received in the protocol. 

To formalize our security proof, we need the following notations:
\begin{itemize}[leftmargin=*] \setlength{\itemsep}{-\itemsep}
\item We use $f(x_1, x_2)$ to denote a function with two variables, where $x_1, x_2\in\{0, 1\}^n$ could be encodings of any mathematical objects, e.g. integers, vectors, matrices, or even functionals. We also use $\pi$ to denote a two-party protocol for computing $f$.

\item The \textit{view} of the $i$th party ($i\in\{1, 2\}$) during the execution of $\pi$ is denoted as $\textbf{view}_i^{\pi}(x_1, x_2, n)$ which can be expanded as $(x_i, \textbf{r}^i, \textbf{m}^i)$, where $x_i$ is the input of $i$th party, $\textbf{r}^i$ is its internal random bits and $\textbf{m}^i$ is the messages received or \textit{derived} by the $i$th party during the execution of $\pi$. Note that $\textbf{m}^i$ includes all the intermediate messages received, all information derived from the intermediate messages, and also the output of $i$th party during the protocol. 

\item A \textit{probability ensemble} $X = \{X(a, n)\}_{a\in\{0, 1\}^*; n\in\mathbb{N}}$ is an infinite sequence of random variables indexed by $a\in\{0, 1\}^*$ and $n\in\mathbb{N}$. In the context of secure multiparty computation, $a$ represents each party's input and $n$ represents problem size. 
\end{itemize}

\begin{definition} Two probability ensembles $X = \{X(a, n)\}_{a\in\{0, 1\}^*; n\in\mathbb{N}}$ and $Y = \{Y(a, n)\}_{a\in\{0, 1\}^*; n\in\mathbb{N}}$ are said to be \textit{computatitionally indistinguishable}, denoted by $X\overset{c}{\equiv} Y$, if for every non-uniform polynomial-time algorithm $D$ and every polynomial $p(\cdot)$, there exists an $N\in\mathbb{N}$ such that for every $a\in \{0, 1\}^*$ and every $n\in \mathbb{N}$,
\begin{eqnarray}
\left|\Pr\{D(X(a,n)) = 1\}-\Pr\{D(Y(a,n)) = 1\}\right|\leq\frac{1}{p(n)}.
\end{eqnarray}
\end{definition}

\begin{definition} \label{def-sim}
Let $f(x_1, x_2)$ be a function. We say a two-party protocol $\pi$ computes $f$ \textit{with information leakage $v_1$ to party 1 and $v_2$ to party 2} where each party is viewed as semi-honest adversaries, if there exist probabilistic polynomial-time algorithms $\mathcal{S}_1$ and $\mathcal{S}_2$ such that
\begin{eqnarray}
\{(\mathcal{S}_1(1^n, x_1, v_1(x_1, x_2)))\}_{x_1, x_2, n}\overset{c}{\equiv}\{(\textbf{view}_1^{\pi}(x_1, x_2, n))\},\\
\{(\mathcal{S}_2(1^n, x_1, v_2(x_1, x_2)))\}_{x_1, x_2, n}\overset{c}{\equiv}\{(\textbf{view}_2^{\pi}(x_1, x_2, n))\},
\end{eqnarray}
where $x_1, x_2\in\{0, 1\}^*$ and $|x_1| = |x_2| = n$.
\end{definition}


\begin{algorithm}[t]
\caption{(SMM-I) Secure matrix multiplication with trusted initializer}\label{algo-trust}
\KwIn {A private matrix $\textbf{X}\in \mathbb{R}^{x\times{}y}$ for $\mathcal{A}$, and a private matrix $\textbf{Y}\in \mathbb{R}^{y\times{}z}$ for $\mathcal{B}$}
\KwOut{A matrix $\textbf{M}\in \mathbb{R}^{x\times{}z}$ for $\mathcal{A}$, and a matrix $\textbf{N}\in \mathbb{R}^{x\times{}z}$ for $\mathcal{B}$, such that $\textbf{M} + \textbf{N} = \textbf{X}\textbf{Y}$}

Trusted Initializer locally generates random matrices $\textbf{U}\in\mathbb{R}^{x\times y}$ and $\textbf{V}\in\mathbb{R}^{y\times{}z}$. Then locally calculates $\textbf{W} = \textbf{U}\textbf{V}$\\
Trusted Initializer locally calculates secret-shares $\textbf{U} = \textbf{U}_1 + \textbf{U}_2$, $\textbf{V} = \textbf{V}_1 + \textbf{V}_2$ and $\textbf{W} = \textbf{W}_1 + \textbf{W}_2$.\\
Trusted Initializer sends $\textbf{U}_1, \textbf{V}_1, \textbf{W}_1$ to $\mathcal{A}$ and $\textbf{U}_2, \textbf{V}_2, \textbf{W}_2$ to $\mathcal{B}$.\\

$\mathcal{A}$ locally calculates secret-shares $\textbf{X} = \textbf{X}_1 + \textbf{X}_2$. Then locally calculates $\textbf{D}_1 = \textbf{X}_1 - \textbf{U}_1$ and $\textbf{E}_1 = \textbf{Y}_1 - \textbf{V}_1$\\
$\mathcal{B}$ locally calculates secret-shares $\textbf{Y} = \textbf{Y}_1 + \textbf{Y}_2$. Then locally calculates $\textbf{D}_2 = \textbf{X}_2 - \textbf{U}_2$ and $\textbf{E}_2 = \textbf{Y}_2 - \textbf{V}_2$\\
$\mathcal{A}$ sends $\textbf{D}_1$ and $\textbf{E}_1$ to $\mathcal{B}$\\
$\mathcal{B}$ sends $\textbf{D}_2$ and $\textbf{E}_2$ to $\mathcal{A}$\\
$\mathcal{A}$ locally calculates $\textbf{M} = \textbf{W}_1 + \textbf{U}_1\textbf{E} + \textbf{D}\textbf{V}_1 + \textbf{D}\textbf{E}$\\
$\mathcal{B}$ locally calculates $\textbf{N} = \textbf{W}_2 + \textbf{U}_2\textbf{E} + \textbf{D}\textbf{V}_2$
\end{algorithm}




\begin{algorithm}[t]
\caption{(SMM-II) Secret matrix multiplication without trusted initializer}\label{algo-ssmm}
\KwIn {A private matrix $\textbf{X}\in \mathbb{R}^{x\times{}y}$ for $\mathcal{A}$, and a private matrix $\textbf{Y}\in \mathbb{R}^{y\times{}z}$ for $\mathcal{B}$}
\KwOut{A matrix $\textbf{M}\in \mathbb{R}^{x\times{}z}$ for $\mathcal{A}$, and a matrix $\textbf{N}\in \mathbb{R}^{x\times{}z}$ for $\mathcal{B}$, such that $\textbf{M} + \textbf{N} = \textbf{X}\textbf{Y}$}

$\mathcal{A}$ and $\mathcal{B}$ locally generate random matrices $\textbf{X}^\prime \in \mathbb{R}^{x\times{}y}$ and $\textbf{Y}^\prime \in \mathbb{R}^{y\times{}z}$ respectively\\
$\mathcal{A}$ locally extracts even columns and odd columns from $\textbf{X}^\prime$, and get $\textbf{X}^\prime_e\in \mathbb{R}^{x\times{}\frac{y}{2}}$ and $\textbf{X}^\prime_o\in \mathbb{R}^{x\times{}\frac{y}{2}}$ respectively\\
$\mathcal{B}$ locally extracts even rows and odd rows from $\textbf{Y}^\prime$, and get $\textbf{Y}^\prime_e\in \mathbb{R}^{\frac{y}{2}\times{}z}$ and $\textbf{Y}^\prime_o\in \mathbb{R}^{\frac{y}{2}\times{}z}$ respectively\\
$\mathcal{A}$ computes $\textbf{X}_1=\textbf{X} + \textbf{X}^\prime$ and $\textbf{X}_2=\textbf{X}^\prime_e + \textbf{X}^\prime_o$, and sends $\textbf{X}_1$ and $\textbf{X}_2$ to $\mathcal{B}$ \\
$\mathcal{B}$ computes $\textbf{Y}_1=\textbf{Y}^\prime - \textbf{Y}$ and $\textbf{Y}_2=\textbf{Y}^\prime_e - \textbf{Y}^\prime_o$, and sends $\textbf{Y}_1$ and $\textbf{Y}_2$ to $\mathcal{A}$ \\
$\mathcal{A}$ locally computes $\textbf{M} = (\textbf{X}+2\textbf{X}^\prime)\textbf{Y}_1 + (\textbf{X}_2+\textbf{X}^\prime_o)\textbf{Y}_2$\\
$\mathcal{B}$ locally computes $\textbf{N} = \textbf{X}_1(2\textbf{Y}-\textbf{Y}^\prime) - \textbf{X}_2(\textbf{Y}_2+\textbf{Y}^\prime_e)$\\
$\mathcal{B}$ sends $\textbf{N}$ to $\mathcal{A}$, and $\mathcal{A}$ calculates $\textbf{M} + \textbf{N}$\\
\Return $\textbf{M} + \textbf{N}$ for $\mathcal{A}$
\end{algorithm}

\subsection{Proof of our protocols}
\begin{theorem}\label{thm-smm1}
Protocol SMM-I (Algorithm \ref{algo-trust}) computes matrix multiplication with no information leakage to both parties.
\end{theorem}
\begin{proof}
Secure matrix multiplication with trusted initializer is a classical protocol, proofs can be found in \textbf{Theorem II.2} in \cite{de2017efficient}.
\end{proof}


\begin{theorem}\label{thm-smm2}
Protocol SMM-II (Algorithm \ref{algo-ssmm}) computes matrix multiplication with information leakage $\textbf{Y}_e-\textbf{Y}_o$ to $\mathcal{A}$ and information leakage $\textbf{X}_e + \textbf{X}_o$ to $\mathcal{B}.$
\end{theorem}
\begin{proof}



\textit{Correctness.} According to Algorithm \ref{algo-ssmm}, we have 
\begin{eqnarray}\small
\label{correctness}
\nonumber
\textbf{M} + \textbf{N} =& (\textbf{X}+2\textbf{X}^\prime)\textbf{Y}_1 + (\textbf{X}_2+\textbf{X}^\prime_o)\textbf{Y}_2 \\
\nonumber
 &+ \textbf{X}_1(2\textbf{Y}-\textbf{Y}^\prime)- \textbf{X}_2(\textbf{Y}_2+\textbf{Y}^\prime_e) \\
 \nonumber
 =& \textbf{X}\textbf{Y}_1 + 2\textbf{X}^\prime\textbf{Y}_1 + \textbf{X}_2\textbf{Y}_2 + \textbf{X}^\prime_o\textbf{Y}_2 \\
 \label{expand}
 &+ 2\textbf{X}_1\textbf{Y}- \textbf{X}_1\textbf{Y}^\prime - \textbf{X}_2\textbf{Y}_2 - \textbf{X}_2\textbf{Y}^\prime_e\\
 \nonumber
 =& \textbf{X}\textbf{Y}^\prime - \textbf{X}\textbf{Y} + 2\textbf{X}^\prime\textbf{Y}^\prime - 2\textbf{X}^\prime\textbf{Y}\\
 \nonumber
 &+ \textbf{X}^\prime_o\textbf{Y}^\prime_e - \textbf{X}^\prime_o\textbf{Y}^\prime_o + 2\textbf{X}\textbf{Y} + 2\textbf{X}^\prime\textbf{Y}\\
 \label{substitute}
 &- \textbf{X}\textbf{Y}^\prime - \textbf{X}^\prime\textbf{Y}^\prime  - \textbf{X}^\prime_e\textbf{Y}^\prime_e - \textbf{X}^\prime_o\textbf{Y}^\prime_e\\
 \label{cancel}
 =& \textbf{X}\textbf{Y} + \textbf{X}^\prime\textbf{Y}^\prime - \textbf{X}^\prime_o\textbf{Y}^\prime_o - \textbf{X}^\prime_e\textbf{Y}^\prime_e\\
 \label{result}
 =&\textbf{X}\textbf{Y}.
\end{eqnarray}
Equation \eqref{substitute} is by substituting $\textbf{X}_1$, $\textbf{X}_2$, $\textbf{Y}_1$, and $\textbf{Y}_2$ in Eq.\eqref{expand} according to line 4 and line 5 in Algorithm \ref{algo-ssmm}. Equation \eqref{cancel} holds by simplifying Eq.\eqref{substitute}. 

The $(i, j)$-th entry of $\textbf{X}^\prime\textbf{Y}^\prime$ is the inner product of the $i$th row of $\textbf{X}^\prime$ and the $j$th column of $\textbf{Y}^\prime$. 
By the  definitions of $\textbf{X}^\prime_o$, $\textbf{X}^\prime_e$, $\textbf{Y}^\prime_o$, and $\textbf{Y}^\prime_e$, the $(i, j)$-th entry of $\textbf{X}^\prime_o\textbf{Y}^\prime_o$ (resp. $\textbf{X}^\prime_e\textbf{Y}^\prime_e$) is the inner product of the odd (resp. even) terms in the $i$-th row of $\textbf{X}^\prime$ and the odd (resp. even) terms in the $j$-th column of $\textbf{Y}^\prime$, so we have $\textbf{X}^\prime\textbf{Y}^\prime = \textbf{X}^\prime_o\textbf{Y}^\prime_o + \textbf{X}^\prime_e\textbf{Y}^\prime_e$ and the last three terms in \eqref{cancel} are cancelled. Thus, the correctness is proved.\\

\textit{Security.} We first give some intuitive discussions on the information disclosure of Algorithm \ref{algo-ssmm}.

Let $\textbf{X}_e$ and $\textbf{X}_o$ be sub-matrices of $\textbf{X}$ constructed by its even columns and odd columns. Similarly let $\textbf{Y}_e$ and $\textbf{Y}_o$ be sub-matrices of $\textbf{Y}$ constructed by its even and odd rows.
As indicated in line 4 of Algorithm \ref{algo-ssmm}, $\mathcal{B}$ has $\textbf{X}_1$, $\textbf{X}_2$ from $\mathcal{A}$. By extracting the even column sub-matrix $\textbf{X}^1_e$ and odd column sub-matrix $\textbf{X}^1_o$ of $\textbf{X}_1$, $\mathcal{B}$ can calculate $\textbf{X}_3 = \textbf{X}^1_e + \textbf{X}^1_o $. Since $\textbf{X}_1 =  \textbf{X} + \textbf{X}^\prime$, we have $\textbf{X}^1_e = \textbf{X}_e + \textbf{X}^\prime_e, \textbf{X}^1_o = \textbf{X}_o + \textbf{X}^\prime_o$. So  $\mathcal{B}$ can compute $\textbf{X}_e + \textbf{X}_o$ by subtracting $\textbf{X}_2$ from $\textbf{X}_3$.  Similar arguments will show that $\mathcal{A}$ can compute $\textbf{Y}_e - \textbf{Y}_o$ as partial information obtained from $\mathcal{B}$. Although $\mathcal{A}$ and $\mathcal{B}$ both have some level of information disclosed as discussed above, their own private data are still unrevealed.

%Similarly, by extracting the even row sub-matrix $\textbf{Y}^1_e$ and odd column sub-matrix $\textbf{Y}^1_o$ of $\textbf{Y}_1$, $\mathcal{A}$ can calculate $\textbf{Y}_3 = \textbf{Y}^1_e - \textbf{Y}^1_o $. Since $\textbf{Y}_1 =  \textbf{Y}^\prime - \textbf{Y}$, we have $\textbf{Y}^1_e = \textbf{Y}^\prime_e - \textbf{Y}_e, \textbf{Y}^1_o = \textbf{Y}^\prime_o -  \textbf{Y}_o$. So  $\mathcal{A}$ can compute $\textbf{Y}_e - \textbf{Y}_o$ by subtracting $\textbf{Y}_3$ from $\textbf{Y}_2$.  

%The above argument shows $\mathcal{B}$ can  learn partial sum of pairwise columns of $\mathcal{A}$'s original data and $\mathcal{A}$ can learn pairwise difference of the rows of $\mathcal{B}$'s original data. However, with this level of information disclosure, both $\mathcal{A}$ and $\mathcal{B}$'s private data are still unrevealed.

To rigorously prove the security level of SMM-II, we adopt the simulation based approach of Definition \ref{def-sim}. Without loss of generality, we first let $\mathcal{A}$ be the adversary and quantify the information leakage to $\mathcal{A}$.
The view of $\mathcal{A}$ in real world contains all information of matrices $\textbf{X}$, $\textbf{X}^\prime$ (including their even and odd column sub-matrices), together with $\textbf{Y}_1$ and $\textbf{Y}_2$. The key point of the proof is to construct a simulator which can reproduce the same distribution of $\textbf{Y}_1$ and $\textbf{Y}_2$. 
The simulator $\mathcal{S}_A$ for $\mathcal{A}$'s view proceeds like this: 
\begin{itemize}
\item[1.] Assume $\mathcal{S}_A$ has $\textbf{Y}_e - \textbf{Y}_o$ as prior knowledge $v_A$;
\item[2.] $\mathcal{S}_A$ generate random matrix $\textbf{Y}^\star \in \mathbb{R}^{y\times{}z}$;
\item[3.] Calculate $\textbf{Y}^\star_2 = (\textbf{Y}^\star_e - \textbf{Y}^\star_o) - (\textbf{Y}_e - \textbf{Y}_o)$.
\end{itemize}

$\textbf{Y}^\star_e$ and $\textbf{Y}^\star_o$ are similarly defined as the even column and odd column sub-matrices of $\textbf{Y}^\star$. We claim that $(\textbf{Y}^\star, \textbf{Y}^\star_2)$ has the same distribution as $(\textbf{Y}_1, \textbf{Y}_2)$, thus being computationally indistinguishable. To see this, we first notice that $\textbf{Y}_1$ is  the difference between a random matrix $\textbf{Y}^\prime$ and a fixed matrix $\textbf{Y}$, which is equally distributed as a random matrix, say $\textbf{Y}^\star$. With this in mind, it can be seen similarly that $\textbf{Y}_e^\star - \textbf{Y}_e$ is equally distributed as $\textbf{Y}_e^\prime$ and $\textbf{Y}_o^\star - \textbf{Y}_o$ is equally distributed as $\textbf{Y}_o^\prime$. Therefore, $\textbf{Y}^\star_2$ is equally distributed as $\textbf{Y}_2$. Moreover, $\mathcal{S}_A$ can reproduce all information of matrices $\textbf{X}$ and $\textbf{X}^\prime$. 

So with additional information of $\textbf{Y}_e - \textbf{Y}_o$, the ideal world simulator $\mathcal{S}_A$ successfully reconstructs the view of $\mathcal{A}$, which is equivalent to say that in the real world, only partial information $\textbf{Y}_e - \textbf{Y}_o$ has been disclosed to $\mathcal{A}$ after running the protocol. 

Similar simulator $\mathcal{S}_B$ can be constructed when assuming $\mathcal{B}$ as the adversary and $\textbf{X}_e + \textbf{X}_o$ as prior knowledge to $\mathcal{B}$. This completes the security proof.

\textit{Complexity.} The computational complexity of SMM-II mainly comes from line 6 and 7, which is $O(x\times y\times z)$. The communication complexity from $\mathcal{A}$ to $\mathcal{B}$ depends on matrices $\textbf{X}_1$ and $\textbf{X}_2$, both of which are of size $O(x\times y)$. 
The communication complexity from $\mathcal{B}$ to $\mathcal{A}$ depends on matrices $\textbf{Y}_1$, $\textbf{Y}_2$, and $\textbf{N}$, which are $O(y\times z)$, $O(y\times z)$, and $O(x\times z)$, respectively, and $O((x+y)\times z)$ in total. 
\end{proof}
%When one of the matrices is sparse, we can slightly modify the secret sharing strategy in Algorithm \ref{algo-ssmm} such that both the computational and communication complexities are reduced accordingly. 
%Without loss of generality, we assume $\textbf{Y}$ is sparse in the sense that for the rows in $\textbf{Y}$ the average number of non-zero entries is $d\ll z$. When generating $\textbf{Y}^\prime$, $\mathcal{B}$ does not make it so dense as in line 1 of Algorithm \ref{algo-ssmm}. 
%The new strategy for generating $\textbf{Y}^\prime$ is as follows:
%
%\For{each row in $\textbf{Y}$}
%{
%	\begin{itemize}
%	\item[1.]generate random numbers for all non-zero entries
%	\item[2.]randomly select $d' \ll z$ entries from the zero entries \\and generate random numbers for these entries 
%	\end{itemize}
%}
%
%
%The value $d'$ is the selected number of non-zero entries of all rows in $\textbf{Y}$, and the above new strategy makes $d'$ small in order to guarantee that the secret shares from $\mathcal{B}$ to $\mathcal{A}$ are sparse. 
%However, as $d'$ becomes smaller, $\mathcal{A}$ would obtain more information on $\textbf{Y}$. 
%An extremal case is $d' = 0$, in which $\mathcal{A}$ can infer the overall sparsity of $Q$. 
%Therefore, a reasonable way is to choose $d' = O(d)$. 
%
%As long as $\textbf{Y}$ is sparse, $\textbf{Y}_1$ and $\textbf{Y}_2$ are both sparse and can be calculated when generating $\textbf{Y}^\prime$. 
%The computational complexity for matrix multiplication decreases to $O(x\times y\times (d + d'))=O(x\times y\times d)$, and the communication complexity from $\mathcal{B}$ to $\mathcal{A}$ decreases to $O(x \times z + y\times(d + d'))=O(x \times z + y\times d)$. Thus both the communication and computational complexity are significantly reduced compared to the general case analysis.
%
%
%We remark that the above discussion on the new secret sharing strategy for sparse matrix exactly satisfy our requirement in SeSoRec. Usually the social matrix $\textbf{S}$ is sparse. When the user social platform $\mathcal{B}$ shares its secrets, it can use the above new strategy to generate its secret shares. 
%Moreover, the choice of $d'$ can be private to $\mathcal{B}$ only so that the user-item interaction platform $\mathcal{A}$ cannot gain more information based on the shares from $\mathcal{B}$.
%%= \textbf{X}_e + \textbf{X}_o + \textbf{X}^\prime_e + \textbf{X}^\prime_o = \textbf{X}_e + \textbf{X}_o + \textbf{X}_2
%
%\subsection{Complexity Analysis of Batch Gradient Descent}
%Now, we analyze the communication and computation complexities of Algorithms \ref{algo-ssrec} and \ref{algo-ssmm}. 
%Recall that $I$ is user number, $J$ is item number, $K$ denotes the dimension of latent factor. 
%
%\textbf{Communication Complexity. }
%The communication cost between two parties only comes from the computation of $\textbf{U}\textbf{D}^T$ and $\textbf{U}\textbf{S}^T$. 
%%The computations of $\textbf{U}\textbf{D}^T$ and $\textbf{U}\textbf{S}^T$ is based on our proposed secure matrix multiplication algorithm, which needs communication between two parties. 
%Let $d$ be the average number of neighbors for each user on platform $\mathcal{B}$. %, and we also randomly select $d'$ zero entries to generate secrets. 
%According to the complexity analysis of SSMM when one matrix is sparse, 
%%suppose the average number of neighbors for each user on platform $\mathcal{B}$ is $|\mathcal{N}|$, 
%the communication cost of $\textbf{U}\textbf{D}^T$ and $\textbf{U}\textbf{S}^T$ from $\mathcal{A}$ to $\mathcal{B}$ are both $O(I\times K)$, and the communication cost of $\textbf{U}\textbf{D}^T$ and $\textbf{U}\textbf{S}^T$ from $\mathcal{B}$ to $\mathcal{A}$ are both $O(K \times I + I\times d)=O(I \times(K+d))$. 
%Since $K$ and $d$ are preset, and $K, d \ll I$, the total communication complexsity is $O(I)$. 
%
%
%\textbf{Computation Complexity. }
%The main computations are lines 3 and 4 in Algorithm \ref{algo-ssrec} and lines 6 and 7 in Algorithm \ref{algo-ssmm}. 
%The time complexity of lines 6 and 7 in Algorithm \ref{algo-ssmm} is $O(I\times K \times d)$, and the time complexity of the lines 3 and 4 in Algorithm \ref{algo-ssrec} is $O(I\times J \times K)$. 
%Since $K, d\ll I, J$, the total time complexity is $O(I\times J)$. 

